Zero-shot Transferable and Persistently Feasible Safe Control for High Dimensional Systems by Consistent Abstraction

Safety is critical in robotic tasks. Energy function based methods have been introduced to address the problem. To ensure safety in the presence of control limits, we need to design an energy function that results in persistently feasible safe control at all system states. However, designing such an energy function for high-dimensional nonlinear systems remains challenging. Considering the fact that there are redundant dynamics in high dimensional systems with respect to the safety specifications, this paper proposes a novel approach called abstract safe control. We propose a system abstraction method that enables the design of energy functions on a low-dimensional model. Then we can synthesize the energy function with respect to the low-dimensional model to ensure persistent feasibility. The resulting safe controller can be directly transferred to other systems with the same abstraction, e.g., when a robot arm holds different tools. The proposed approach is demonstrated on a 7-DoF robot arm (14 states) both in simulation and real-world. Our method always finds feasible control and achieves zero safety violations in 500 trials on 5 different systems.

==> conclusion.tex <==
% In conclusion, we propose a new method called abstract safe control that enables ensuring persistent feasibility for high dimensional systems by consistent system abstraction. 
Our method provides a promising solution for ensuring safety in high-dimensional robotic tasks, with potential applications in various domains. In the future, we will explore how to derive the analytical upper bound of $\dot M_{max}$ to avoid the sampling-based estimation.
% ~\footnote{The appendix can be found at https://arxiv.org/abs/2209.06896\label{arxiv}}
